Bringing Federated Learning to Space

As Low Earth Orbit (LEO) satellite constellations rapidly expand to hundreds and thousands of spacecraft, the need for distributed on-board machine learning becomes critical to address downlink bandwidth limitations. Federated learning (FL) offers a promising framework to conduct collaborative model training across satellite networks. Realizing its benefits in space naturally requires addressing space-specific constraints, from intermittent connectivity to dynamics imposed by orbital motion. This work presents the first systematic feasibility analysis of adapting off-the-shelf FL algorithms for satellite constellation deployment. We introduce a comprehensive "space-ification" framework that adapts terrestrial algorithms (FedAvg, FedProx, FedBuff) to operate under orbital constraints, producing an orbital-ready suite of FL algorithms. We then evaluate these space-ified methods through extensive parameter sweeps across 768 constellation configurations that vary cluster sizes (1-10), satellites per cluster (1-10), and ground station networks (1-13). Our analysis demonstrates that space-adapted FL algorithms efficiently scale to constellations of up to 100 satellites, achieving performance close to the centralized ideal. Multi-month training cycles can be reduced to days, corresponding to a 9x speedup through orbital scheduling and local coordination within satellite clusters. These results provide actionable insights for future mission designers, enabling distributed on-board learning for more autonomous, resilient, and data-driven satellite operations.

==> Content/Z_Appendicies.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\appendices{}              % note there is no {} to put a title. Each appendix has its own title
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% For a single appendix, use the \appendix{} keyword and do not use the \section command.

\section{More Information}        % first appendix
%%%%%%%%%%%%%%%%%%%%%%%%%%
This is the first appendix. 

\subsection{Comments}
If you have only one appendix, use the ``appendix'' keyword.

\subsection{More Comments}
Use section and subsection keywords as usual.


\section{Summary of Format Requirements}    % second appendix - added 4/10/2025 to be consistent with word template
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textit{Paper size: }8.5 x 11 inch

 \textit{Number of pages}: 6–20

 \textit{Margins}\\
\hspace*{2em}Top and bottom: 0.75 inch\\
\hspace*{2em}Left and right: 0.75 inch

 \textit{Columns}\\
\hspace*{2em}Number of columns: 2\\
\hspace*{2em}Space between: 0.25 inch

 \textit{Font}: Times Roman 10 pt regular, unless otherwise noted

 \textit{Text}\\
\hspace*{2em}Line spacing: Single\\ 
\hspace*{2em}Space after paragraph: 10 pt\\ 
\hspace*{2em}Paragraph indent: None \\
\hspace*{2em}Justification: Left \& right\\

 \textit{Title}\\
\hspace*{2em}20 pt bold, upper \& lower case, initial caps on all words \hspace*{3em}except articles, conjunctions and prepositions\\
\hspace*{2em}Centered on the full-page width\\
\hspace*{2em}Maximum length 100 characters\\

 \textit{Author(s)}\\
\hspace*{2em}10 pt bold, upper and lower case\\
\hspace*{2em}Centered on the full-page width\\
\hspace*{2em}Name, affiliation, postal address, phone number, and\\\hspace*{3em}e-mail\\
\hspace*{2em}No degrees or titles, except military rank\\

 \textit{Abstract: }9 pt bold

 \textit{Acronyms}: Define acronyms on first usage

 \textit{Page numbers}: Bottom center of each page, including first page

 \textit{Footnotes}: 8 pt regular

 \textit{Headings}\\
\hspace*{2em}Spacing before major or subheadings: Double space\\
\hspace*{2em}Spacing after major or subheadings: 1.5 space\\
\hspace*{2em}Major headings: 12 pt small caps, bold, centered\\
\hspace*{2em}Subheadings: 10 pt italic, flush left, separate line\\
\hspace*{2em}Subsubheadings: 10 pt italic, run into paragraph with\\ 
\hspace*{3em}em dash\\

 \textit{Headers and Footers}\\
\hspace*{2em}No headers\\
\hspace*{2em}Footers used for page numbers and\\
\hspace*{3em}Copyright notice on page 1\\

 \textit{Equations}\\
\hspace*{2em}Centered in column\\
\hspace*{2em}Equation numbers in parentheses, flush right\\
\hspace*{2em}Include special fonts with the paper.\\

 \textit{Figures and Tables}\\
\hspace*{2em}Captions and titles: 10 pt bold\\
\hspace*{2em}Figure captions: Centered directly below figures\\
\hspace*{2em}Table titles: Centered directly above tables\\
\hspace*{2em}Scanned images: 300 dpi JPEG\\

 \textit{References}\\
\hspace*{2em}List references at end of paper.\\
\hspace*{2em}References numbers: In square brackets [ ]\\

 \textit{Biography}\\
\hspace*{2em}Each author's name in bold italic\\
\hspace*{2em}Brief biography in 10 pt italic\\
\hspace*{2em}Photo of each author\\


==> figures/heatmaps_fedavg.tex <==

\begin{figure*}[!ht]

    \begin{subfigure}{\textwidth}
    \centering
    \includegraphics[trim={7cm 0 7cm 0},clip,scale = 0.25]{figures/acc/fedAvgSat_acc.png}
    \caption{FedAvg with space-ification, accuracy heatmaps}
    \label{fig:fedavg:acc_1}
    \end{subfigure}
    \begin{subfigure}{\textwidth}
    \centering
    \includegraphics[trim={7cm 0 7cm 0},clip,scale = 0.25]{figures/dur/fedAvgSat_10_duration.png}
    \caption{FedAvg with space-ification, round duration heatmaps}
    \label{fedavg10:duration_1}
    \end{subfigure}
    \begin{subfigure}{\textwidth}
    \centering
    \includegraphics[trim={7cm 0 7cm 0},clip,scale = 0.25]{figures/idle/fedAvgSat_10_iavg.png}
    \caption{FedAvg with space-ification, idle time heatmaps}
    \label{fedavg10:iavg_1}
    \end{subfigure}
    
    \caption{An example set of heatmaps for FedAvg with space-ification, outlining performances in accuracy, FL round durations, and idle time. Even on the most barebones FL algorithm, we see that with large enough constellation sizes and ground station networks, enough opportunities for access windows can be made to reach convergence. Proper comparisons against performance of other algorithms can be found in the appendix, highlighting the importance of the augmentations on FL algorithm performance. }\label{fig:fedavgheatmap}
\end{figure*}


==> tables/autoflsat_clusters.tex <==
%%%TODO FOR GRACE: The #s of rounds don't turly make senes

\setlength{\tabcolsep}{30pt}

\begin{table*}[htp]
  \setlength{\tabcolsep}{0.3\tabcolsep}
\centering
\resizebox{0.9\linewidth}{!}{%
\begin{tabular}{cc|cccc}
\toprule
\textbf{\# of Clusters} & \textbf{\# of Epochs} & \textbf{Accuracy} & \textbf{Round Duration} & \textbf{Idle Time}& \textbf{Total Training Time} \\ \midrule
4 & 20 & 83.3\% & 12.1 min & 10.3 min& 20.6 Hours \\ 
4 & 50 & 83.01\%  & 11.93 min & 10.2 min & 21.28 Hours \\
4 & 100 & 82.5\%  & 12.3 min & 10.32 min & 28.1 Hours \\ \midrule
3 & 20 & 82.8\%  & 9.53 min & 8.4 min & 28 Hours\\
3 & 50 & 81.4\% & 9.4 min & 8.3 min & 22 Hours\\
3 & 100 & 82.2\%  & 9.3 min & 8.4 min & 18.79 Hours\\ \midrule
2 & 20 & 82.1\% & 4.5 min & 3.26 min & 14.3 Hours\\
2 & 50 & 82.5 \% & 4.6 min & 3.01 min & 15.2 Hours\\
2 & 100 & 81\% & 4.6 min & 2.6 min & 20.99 Hours\\


\bottomrule
\end{tabular}
}
\caption{Experiments of \textit{AutoFLSat} trained on the FEMNIST dataset, varying both the \#s of clusters and \#s of epochs tested. Values of the accuracy, round duration, idle time, and total training time are outlined. With increases in the \#s of clusters in the constellation, there is definitely an increase in idle time spent trying to accumulate every cluster's global model. These increases in idle time take up a large portion of the round duration, which may scale with the size of the constellation. The accuracy is able to be met at a reasonable time frame for each constellation setup, but a clear connection with accuracy percentages and constellation setups are not established.}
\label{tab:autoFLSat}
\end{table*}

==> tables/autoflsat_comparisons.tex <==

\setlength{\tabcolsep}{30pt}

\begin{table}[htbp]
  \setlength{\tabcolsep}{0.3\tabcolsep}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{c|ccc} %|p{3cm}
\toprule
\textbf{FL Algorithm} & \textbf{Dataset} & \textbf{Accuracy} & \textbf{Training Time} \\ \midrule

AutoFLSat (4 Clusters) & FEMNIST & 83.01\% & 21.28 hours \\ 
NomaFedHAP & non-IID MNIST & 82.73\% & 24 hours \\ 
FedLEO & non-IID MNIST & 84.69\% & 36 hours \\ 
FedSat & non-IID MNIST & 85.15\% & 24 hours \\ 
FedSpace & non-IID MNIST & 52.67\% & 72 hours \\ 
\midrule
AutoFLSat (4 Clusters) & CIFAR-10 & 82.46\% & 15.6 Hours \\ 
NomaFedHAP & CIFAR-10 & 77.36\% & 24 hours \\ 
FedLEO & CIFAR-10 & 73.26\% & 36 hours \\ 
FedSat & CIFAR-10 & 81.18\% & 24 hours \\ 
FedSpace & CIFAR-10 & 39.41\% & 72 hours \\

\bottomrule
\end{tabular}
}

\vspace*{3mm}
\caption{Evaluation of \textit{AutoFLSat} with other leading FL in space algorithms, specifically trained on the FEMNIST and CIFAR-10 datasets. These two datasets have been used as a standard benchmark for performance assessment across, with metrics of final performance accuracy and total training time being contrasted against. For accuracy, \textit{AutoFLSat} is on the higher end of convergence percentages compared to the other FL in Space methods. The larger distinguishing factor however, is the faster training time found to reach the model accuracy convergence listed.}
\label{tab:autoFLSat_compares}
\end{table}

==> tables/eurosat.tex <==

\setlength{\tabcolsep}{30pt}

\begin{table*}[htp]
  \setlength{\tabcolsep}{0.3\tabcolsep}
\centering
\resizebox{0.75\linewidth}{!}{%
\begin{tabular}{c|ccccc}
\toprule
\textbf{\# of Clusters} & \textbf{Accuracy} & \textbf{Round Duration}& \textbf{Idle Time}& \textbf{Total Training Time} \\ \midrule
4 & 83.5\% & 12.4 min & 10.23 min & 14.1 Hours \\ \midrule
3 & 80.5\% & 9.6 min & 8.34 min & 11.2 Hours\\\midrule
2 & 82.1\% & 4.5 min & 2.6 min & 6.4 Hours\\


\bottomrule
\end{tabular}
}

\vspace*{3mm}
\caption{Experiments of \textit{AutoFLSat} trained on the EUROSAT dataset, varying both the \#s of clusters and \#s of epochs tested. Values of the accuracy, \# of rounds trained on, round duration, idle time, and total training time are outlined. Similar increases in idle time and round duration is found from the increase of \# of clusters as found in the FEMNIST dataset. However, speedy convergence is reached for image classification training on the EUROSAT satellite image patch collection, which gives promising indications of \texttt{AutoFLSat} providing proper convergence when trained on realistic data.}
\label{tab:eurosatautoflsat}
\end{table*}

==> tables/groundstations.tex <==

\begin{table}[htbp]
\centering
\footnotesize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.2}
\resizebox{0.95\linewidth}{!}{%
\begin{tabular}{c l l}
\toprule
\textbf{\# Ground Stations} & \textbf{Names} & \textbf{Coordinates (Lat, Lon)} \\ \midrule
\multirow{1}{*}{1}  & Sioux Falls & (43.55, -96.72) \\ \hline
\multirow{1}{*}{2}  & Sanya & (18.25, 109.5) \\ \hline
\multirow{1}{*}{3}  & Johannesburg & (-26.2, 28.03) \\ \hline
\multirow{2}{*}{5}  & Cordoba & (-31.4, -64.18) \\ 
                     & Tromso & (69.65, 18.95) \\ \hline
\multirow{5}{*}{10} & Kashi & (39.1, 77.2) \\
                     & Beijing & (39.9, 116.4) \\
                     & Neustrelitz & (53.1, 13.1) \\
                     & Parepare & (-2.99, 119.8) \\
                     & Alice Springs & (-25.1, 133.9) \\ \hline
\multirow{3}{*}{13} & Fairbanks & (64.8, -147.7) \\
                     & Prince Albert & (53.2, -105.7) \\
                     & Shadnagar & (17.4, 78.5) \\
\bottomrule
\end{tabular}
}
\caption{Ground station names and latitude/longitude coordinates used in different experimental sweeps. Each row shows one station, with the left column spanning the total number of stations for that configuration.}
\label{tab:groundStationNamesCoords}
\end{table}


==> tables/table_autofl_Experiments.tex <==

\setlength{\tabcolsep}{30pt}

\begin{table*}[htp]

  \setlength{\tabcolsep}{0.3\tabcolsep}
\centering
\resizebox{0.8\linewidth}{!}{%
\begin{tabular}{cccccc}
\toprule
\textbf{FL Alg} & \textbf{Communication Method} & \textbf{Dataset} &  \textbf{Epochs} &\textbf{Clusters} \\ \midrule
AutoFLSat & Intra/Inter Sat Links & FEMNIST & $20,50,100,250$ & $2,3,4$ \\

AutoFLSat & Intra/Inter Sat Links & CIFAR-10 & $1,3,5,10$ & $2,3,4$ \\

AutoFLSat & Intra/Inter Sat Links & EUROSAT & $1,3,5,10$ &$2,3,4$ \\




\bottomrule
\end{tabular}
}
\caption{\textit{AutoFLSat} specific parameter configuration settings, testing differences in \# of clusters, datasets, and epochs of training in each round. Three datasets are tested against, FEMINIST, CIFAR-10, and EUROSAT, with \#s of clusters in the constellation ranging from 2, 3, and 4. Varying epochs suitable for each type of training dataset are tested as well. There are 10 satellites per cluster.}
\label{tab:autoflConfigs}
\end{table*}

==> tables/table_classes_sat_hardware.tex <==
\begin{table*}[!tb]
    \centering
    \footnotesize
    \caption{Classes of satellite hardware.}
    \begin{tabular}{ l  c cccc c c }
        \toprule
         & & \multicolumn{2}{c}{\textbf{Communications}} \\
         \cmidrule(lr){3-4}
         \textbf{Class} & \textbf{Compute} & \textbf{F-Band} & \textbf{Data Rate} & \textbf{OAP} & \textbf{Cost (Est.)} & \textbf{CubeSat Size} \\
        \midrule
         Low-end & - & - & - & - & - \\   
        \midrule
         Medium-end & - & - &  - & - & - \\  
        \midrule
         High-end & - & - &  - & - & - \\  
        \bottomrule
    \end{tabular}
     \label{tab:satellite_hardware_categories}
\end{table*}

==> tables/table_experiments.tex <==
\begin{table}[htbp]
    \renewcommand{\arraystretch}{1.0}
    \centering
    \scriptsize % smaller font
    \setlength{\tabcolsep}{4pt} % tighter spacing
    \begin{tabular}{l l c c c}
    \toprule
    \textbf{FL Alg} & \textbf{Extension} & \textbf{Clusters} & \textbf{Sats/Cluster} & \textbf{Ground Stations} \\ 
    \midrule
    FedAvg  & Base      & $1,2,5,10$ & $1,2,5,10$ & $1,2,3,5,10,13$ \\
            & Schedule  & $1,2,5,10$ & $1,2,5,10$ & $1,2,3,5,10,13$ \\
            & IntraCC   & $1,2,5,10$ & $1,2,5,10$ & $1,2,3,5,10,13$ \\
    \midrule
    FedProx & Base      & $1,2,5,10$ & $1,2,5,10$ & $1,2,3,5,10,13$ \\
            & Schedule  & $1,2,5,10$ & $1,2,5,10$ & $1,2,3,5,10,13$ \\
            & Sched V2  & $1,2,5,10$ & $1,2,5,10$ & $1,2,3,5,10,13$ \\
            & IntraCC   & $1,2,5,10$ & $1,2,5,10$ & $1,2,3,5,10,13$ \\
    \midrule
    FedBuff & Base      & $1,2,5,10$ & $1,2,5,10$ & $1,2,3,5,10,13$ \\
    \bottomrule
    \end{tabular}
    \caption{Parameter configurations tested across space-ified FL algorithms (\textit{FedAvg}, \textit{FedProx}, \textit{FedBuff}). Sweeps cover clusters, satellites per cluster, and ground stations, evaluated on FEMNIST, leading to 768 total tested configurations.}
    \label{tab:clflConfigs}
\end{table}

